M-IHS: An Accelerated Randomized Preconditioning Method Avoiding Costly Matrix Decompositions

Momentum Iterative Hessian Sketch (M-IHS) techniques, a group of solvers for large scale regularized linear Least Squares (LS) problems, are proposed and analyzed in detail. Proposed M-IHS techniques are obtained by incorporating the Heavy Ball Acceleration into the Iterative Hessian Sketch algorithm and they provide significant improvements over the randomized preconditioning techniques. By using approximate solvers along with the iterations, the proposed techniques are capable of avoiding all matrix decompositions and inversions, which is one of the main advantages over the alternative solvers such as the Blendenpik and the LSRN. Similar to the Chebyshev semi-iterations, the M-IHS variants do not use any inner products and eliminate the corresponding synchronization steps in hierarchical or distributed memory systems, yet the M-IHS converges faster than the Chebyshev Semi-iteration based solvers. Lower bounds on the required sketch size for various randomized distributions are established through the error analyses. Unlike the previously proposed approaches to produce a solution approximation, the proposed M-IHS techniques can use sketch sizes that are proportional to the statistical dimension which is always smaller than the rank of the coefficient matrix. The relative computational saving gets more significant as the regularization parameter or the singular value decay rate of the coefficient matrix increase.

==> files/definitions.tex <==
%%widebar
\makeatletter
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{%
  \begingroup
  \def\mathaccent##1##2{%
    \rel@kern{0.8}%
    \overline{\rel@kern{-0.8}\macc@nucleus\rel@kern{0.2}}%
    \rel@kern{-0.2}%
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \macc@nested@a\relax111{#1}%
  \endgroup
}


\newcommand{\ones}{\mathbb{1}}
\newcommand{\reals}[1]{{\mathbb{R}^{#1}}}
\newcommand{\compls}[1]{{\mathbb{C}^{#1}}}
\newcommand{\integers}[1]{{\mathbb{Z}^{#1}}}
\newcommand{\realss}[2]{{\mathbb{R}^{#1 \times #2}}}
\newcommand{\complss}[2]{{\mathbb{C^{#1 \times #2}}}}
\newcommand{\symm}[2]{{\mathbb{S^{#1 \times #2}}}}  % symmetric matrices
\DeclareMathOperator{\spans}{\text{{span}}}
\DeclareMathOperator{\nnz}{\text{{nnz}}}
%\newcommand{\nullspace}{{\mathcal N}}
%\newcommand{\range}{{\mathcal R}}
%\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\tr}[1]{\mathsf{tr}\left(#1\right)}
%\newcommand{\diag}{\mathop{\bf diag}}
%\newcommand{\card}{\mathop{\bf card}}
%\newcommand{\rank}{\mathop{\bf rank}}
%\newcommand{\conv}{\mathop{\bf conv}}
%\newcommand{\prox}{\mathbf{prox}}

\newcommand{\expect}[1]{\mathop{\mathbb{E}}\left[#1\right]}
\newcommand{\expectt}[2]{\mathbb{{ E}}_{#1}\left[#2\right]}
%\newcommand{\Prob}{\mathop{\bf Prob}}
%\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
%\newcommand{\dist}{\mathop{\bf dist{}}}
%\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\argmax}{\mathop{\rm argmax}}
%\newcommand{\epi}{\mathop{\bf epi}} % epigraph
%\newcommand{\Vol}{\mathop{\bf vol}}
%\newcommand{\dom}{\mathop{\bf dom}} % domain
%\newcommand{\intr}{\mathop{\bf int}}
%\newcommand{\sign}{\mathop{\bf sign}}

%\newcommand{\cf}{{\it cf.}}
%\newcommand{\eg}{{\it e.g.}}
%\newcommand{\ie}{{\it i.e.}}
%\newcommand{\etc}{{\it etc.}}

\newcommand{\swrite}[2]
{
\underset{#2}{\mbox{#1 }} 
}

\newcommand{\lscost}[2]
{
\left\|{#1}\right\|_{#2}
}
\newcommand{\x}[1]
{
x^{#1}
}

\newcommand{\K} 
{
\mathcal{K}
}
\newcommand{\nf}[3]
{
\nabla^{#1}f\left(#2\right)^{#3}
}

\newcommand{\Se} 
{
\mathcal{S}^{\text{d-1}}
}

\newcommand{\KS} 
{
\K \cap \Se
}
\newcommand{\W} 
{
\mathcal{W}
}

\newcommand{\Y} 
{
\mathcal{Y}
}
\newcommand{\D} 
{
\mathcal{D}
}
\newcommand{\prob}[2]{\mathbb{{ P}}_{#1}\left(#2\right)}
\newcommand{\sd}{\mathsf{sd}_\lambda}
%\newcommand{\ff}[1]{{\fontfamily{lmtt}\selectfont#1}}
\newcommand{\ff}[1]{{#1}}
\newcommand{\xls} 
{
\mathbf{x}_{\text{LS}}
}
\newcommand{\dof}{\mathsf{dof}}
\newcommand{\sdd}[1]{\mathsf{sd}_{{\lambda}^{#1}}}
\newcommand{\sddd}[1]{\mathsf{sd}_{{\lambda}_{#1}}}
\newcommand{\V} 
{
\mathbb{V}
}
\DeclareMathOperator{\diag}{\bf diag}

==> sections/algorithms.tex <==
The \ff{M-IHS} is obtained by combining the IHS technique with the Heavy Ball Acceleration. The IHS technique iteratively minimizes the quadratic objective in \cref{eq:intro} by performing the following updates:
\begin{align*}
    x^{i+1} &= \swrite{argmin }{x\in\reals{d}} \lscost{S_iA(x - x^i)}{2}^2 + \lambda\lscost{x-x^i}{2}^2 + 2\langle \nabla f(x^i),\ x \rangle, \\
    &= x^i + (A^TS_i^TS_iA + \lambda I_d)^{-1}\left(A^T(b - Ax^i) - \lambda x^i\right).
\end{align*}
In all iterations, the same sketching matrix can be used by adding a proper step size and the convergence can be accelerated by an additional momentum term, which give raise to the following \ff{M-IHS} iterations:
\begin{align}
    \Delta x^i &= \swrite{argmin }{x\in\reals{d}} \lscost{SAx}{2}^2 + \lambda\lscost{x}{2}^2 + 2\left\langle \nabla f(x^i), \ x\right\rangle, \label{eq:mihs1}\\
    x^{i+1}&= x^i + \alpha_i\Delta x^i + \beta_i \left(x^i - x^{i-1}\right). \nonumber
\end{align}
If we restrict our attention to the fixed parameters, the optimal momentum parameters $\alpha$ and $\beta$, that maximize the convergence rate, can be estimated by using random matrix theory as completely independent of spectral properties of the coefficent matrix $A$. Here, the linear system is assumed to be strongly over-determined, i.e., $n\gg d$, but  by using the dual problem, the theory can be easily extended to the strongly under-determined case of $d\gg n$ as well \cite{ref:boyd_cvx}. A dual of the problem in \cref{eq:intro} is
\begin{equation}
    \nu^* = \swrite{argmin }{\nu\in\reals{n}} \underbrace{\frac{1}{2}\lscost{A^T\nu}{2}^2 + \frac{\lambda}{2}\lscost{\nu}{2}^2 - \langle b,\ \nu\rangle}_{g(\nu)}, \label{eq:intro_dual}
\end{equation}
and the relation between the solutions of the primal and dual problem is
\begin{equation}
    \nu^* = (b - Ax^*)/\lambda \Longleftrightarrow x^* = A^T\nu^*. \label{eq:dual_relation}
\end{equation}
The dual problem in \cref{eq:intro_dual} can be minimized by using the same approach as the \ff{M-IHS}:
\begin{align}
    \Delta \nu^i &= \swrite{argmin }{\nu\in\reals{n}}\lscost{SA^T\nu}{2}^2 +\lambda\lscost{\nu}{2}^2 + 2\left\langle \nabla g(\nu^i),\ \nu\right\rangle, \label{eq:dual_mihs1}\\
    \nu^{i+1} &= \nu^{i} + \alpha \Delta\nu^i + \beta\left(\nu^i - \nu^{i-1}\right),\nonumber
\end{align}
and the solution of the primal problem can be obtained through the relation in \cref{eq:dual_relation}. We refer to this algorithm as \ff{Dual M-IHS}. The convergence rates of the \ff{M-IHS} and \ff{Dual M-IHS} solvers together with the necessary condition are stated in the \cref{lemma:mihs_conv} below.
\begin{theorem}\label{lemma:mihs_conv}
Let $A$ and $b$ be the given data in \cref{eq:setup}; $x^*\in\reals{d}$ and $\nu^*\in\reals{n}$ are as in \cref{eq:intro} and \cref{eq:intro_dual}, respectively. Let $U_1 \in\realss{\max(n,d)}{\min(n,d)}$ consists of the first $n$ rows of an orthogonal basis for $\begin{bmatrix}A\\\sqrt{\lambda}I_d\end{bmatrix}$ if the problem is  over-determined, and consists of the first $d$ rows of an orthogonal basis for $\begin{bmatrix}A^T\\\sqrt{\lambda}I_n\end{bmatrix}$ if the problem is under-determined. Let the sketching matrix $S\in\realss{m}{\max(n,d)}$ be drawn from a distribution $\D$ such that
\begin{equation}
    \prob{S\sim\D}{\lscost{U_1^TS^TSU_1 - U_1^TU_1}{2} \geq \epsilon} < \delta, \quad \epsilon \in(0,1) \label{condition:1}.
\end{equation}
Then, the {\normalfont\ff{M-IHS}} applied on \cref{eq:intro} and the {\normalfont\ff{Dual M-IHS}} applied on \cref{eq:intro_dual} with fixed momentum parameters
\begin{equation*}
    \beta^* = \left(\frac{\sqrt{1+\epsilon} - \sqrt{1-\epsilon}}{\sqrt{1+\epsilon} + \sqrt{1-\epsilon}}\right)^2, \quad\quad \alpha^* = \left(1 - \beta^*\right)\sqrt{1 - \epsilon^2},
\end{equation*}
converge to the optimal solutions, $x^*$ and $\nu^*$, respectively, at the following rate\footnote{$\sqrt{\beta} = \frac{\epsilon}{1 + \sqrt{1 - \epsilon^2}}$} with probability at least $1-\delta$:
\begin{align*}
    \lscost{x^{i+1} - x^{*}}{D^{-1}} \leq \frac{\epsilon}{1 + \sqrt{1 - \epsilon^2}} \lscost{x^i - x^*}{D^{-1}}, \\ 
    \lscost{\nu^{i+1} - \nu^{*}}{D^{-1}} \leq \frac{\epsilon}{1 + \sqrt{1 - \epsilon^2}} \lscost{\nu^i - \nu^*}{D^{-1}},
\end{align*}
where $D^{-1}$ is the diagonal matrix whose diagonal entries are $\sqrt{\sigma_i^2 + \lambda}$ and $\sigma_i$ is the $i$-th singular value of $A$.
\end{theorem}
The proof of \cref{lemma:mihs_conv} can be found in \cref{proof:lemma_conv}. The \cref{lemma:mihs_conv} is valid as well for the un-regularized case of $\lambda = 0$ as mentioned in \cref{proof:no_reg}. When the necessary conditions are met, the number of iterations needed for both algorithms to reach a certain level of accuracy is stated in the following corollary.
\begin{corollary}\label{corollary:iter}
For some $\epsilon\in(1, 1/2)$ and arbitrary $\eta$, if the sketching matrix meets the condition in \cref{condition:1} and the fixed momentum parameters are chosen as in \cref{lemma:mihs_conv}, then the {\normalfont\ff{M-IHS}} and the {\normalfont\ff{Dual M-IHS}} obtain an $\eta$-optimal solution approximation in $\ell2$-norm with total of
$$N = \left\lceil \frac{\log(\eta)\log(C)}{\log(\epsilon) - \log(1 + \sqrt{1 - \epsilon^2})}\right\rceil$$
iterations where the constant $C$, that is defined as $C = \sqrt{\kappa(A^TA+\lambda I_d)}$ for the {\normalfont\ff{M-IHS}} and $C = \kappa(A)\sqrt{\kappa(AA^T+\lambda I_n)}$ for the {\normalfont\ff{Dual M-IHS}}, can be removed if the semi-norm in \cref{lemma:mihs_conv} is used as the solution approximation metric instead of $\ell2$ norm.
\end{corollary}
\Cref{corollary:iter} is an immediate result of \cref{lemma:mihs_conv}. Some possibilities for the distributions satisfying the condition in \cref{condition:1} of \cref{lemma:mihs_conv} are given in \cref{corollary:sketch}.
\begin{lemma} \label{corollary:sketch}
The condition in \cref{lemma:mihs_conv} is satisfied if the sketching matrix $S$ is in one of the following types:
\begin{enumerate}[label=(\roman*)]
    \item\label{item1} Sparse Subspace Embedding \cite{ref:w14_sketching_asatool} with single nonzero element in each column, sketch size
    $$m =\Omega\left( \mathbf{sd}_\lambda(A)^2/(\epsilon^2\delta)\right)$$
    and $SA$ is computable in $O(\mathbf{nnz}(A))$;
    \item\label{item2} Sparse Subspace Embedding with $\alpha> 2$, $\delta<1/2$, $\epsilon<1/2$,
    $$s = \Omega(\log_\alpha(\sd(A)/\delta)/\epsilon)$$
    non-zero elements in each column \cite{ref:kn14_sparser_jl, ref:nn13_osnap}, size    
    $$m = \Omega(\alpha\cdot\sd(A)\log(\sd(A)/\delta)/\epsilon^2)$$
    and $SA$ is computable in $O(s\cdot\mathbf{nnz}(A))$;
    \item\label{item3} SRHT sketching matrix \cite{ref:cnw15_optimal_stable_rank, ref:ihs} with size
    $$m= \Omega\left(\left(\mathbf{sd}_\lambda(A)+\log(1/\epsilon\delta)\log(\mathbf{sd}_\lambda(A)/\delta)\right)/\epsilon^{2}\right)$$
    and $SA$ is computable in $O(nd\log(m))$;
    \item\label{item4} Sub-Gaussian sketching matrix \cite{ref:pilanci1, ref:cnw15_optimal_stable_rank} with size
    $$m = \Omega(\sd(A)/\epsilon^2)$$ 
    and $SA$ is computable in $O(ndm)$.
\end{enumerate}
\end{lemma}
The proof of \cref{corollary:sketch} can be found in \cref{proof:cor_sketch}. \Cref{corollary:sketch} suggests that in order to satisfy the condition in \cref{lemma:mihs_conv}, the sketch size can be chosen proportional to the statistical dimension of the problem which can be considerably smaller than the rank. Moreover, to obtain a solution approximation, we do not need the second condition in Lemma 11 of \cite{ref:acw16_sharper}, hence we obtained slightly better results for the sparse subspace embeddings in item $(i)$ and $(ii)$ of \cref{corollary:sketch}. In \cref{corollary:empirical}, we obtained substantially simplified empirical versions of the convergence rate, momentum parameters and required sketch size by using the MP Law \cite{ref:edelman2} and approximating the filtering coefficients of Tikhonov regularization with binary coefficients. \Cref{corollary:empirical} suggests that the ratio between the statistical dimension and sketch size determines the convergence rate of the proposed algorithms, which interestingly seems valid even for the sketch matrices with single non-zero element in each column.
\begin{corollary}\label{corollary:empirical}
Let the entries of sketching matrix be independent, zero mean, unit variance and that have bounded higher order moments. If the Truncated SVD regularization with truncation parameter $\lceil \sd(A) \rceil$ is used, then the {\normalfont\ff{M-IHS}} and {\normalfont\ff{Dual M-IHS}} with the following momentum parameters
\begin{equation*}
    \beta = \frac{\sd(A)}{m}, \quad\quad \alpha = (1- \beta)^2
\end{equation*}
will converge to the optimal solutions $x^*$ and $\nu^*$ respectively with a convergence rate of $\sqrt{\beta}$ as $m\to \infty$ while $\min(n,d)/m$ remains constant. Any sketch size $m > \sd(A)$ can be chosen to obtain an $\eta$-optimal solution approximation at most $\frac{\log(\eta)}{\log(\sqrt{\beta})}$ iterations. 
\end{corollary}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfile{demos/fig_convergence}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Although MP law provides bounds for the singular values of the sketching matrix $S$ in asymptotic regime, i.e., as $m\to\infty$; these bounds become very good estimators of the actual bounds when $m$ takes finite values, as demonstrated in \cref{fig:convergence}.  In \cref{fig:convergence_1}, $A\in\realss{32768}{1000}$ with $\kappa(A) = 10^8$ is generated as described in \cref{sec:ex_setup}. In \cref{fig:convergence_2}, $A\in\realss{24336}{1296}$ is generated by using \textit{sprand} command of MATLAB. We first create a sparse matrix with size $\Tilde{A}\in\realss{20}{6}$ and sparsity $15\%$, then the final form is obtain by taking $A = \Tilde{A}^{\otimes 4}$ and deleting the all zero rows. The final form $A$ has sparsity ratio $0.1\%$ and condition number $\kappa(A) = 10^7$. The noise level is set to = $1\%$ in both experiments and the resulting statistical dimensions are $119$ and $410$ respectively. The rate of $\sqrt{\beta}$ in \cref{corollary:empirical} creates a remarkable fit to the numerical convergence rate of the \ff{M-IHS} variants when the momentum parameters given in \cref{corollary:empirical} are used even for the Tikhonov regularization. This is because the sigmoid-like filtering coefficients in the Tikhonov regularization can be thought of as the smoothed version of the binary coefficients in the TSVD solution and therefore the binary coefficients constitute a good approximation for the filtering coefficients of the Tikhonov regularization.

\begin{remark}
The momentum parameters given in \Cref{corollary:empirical} minimizes the convergence rate when the statistical dimension is known. If $\beta$ is chosen larger than the ratio $\sd(A)/m$ with $\alpha = (1-\beta)^2$, then the convergence rate will be still $\sqrt{\beta}$ since the dynamical system will be still in the under-damped regime. An overestimated statistical dimension value can be cheaply found by using Hutchinson-like estimators together with the sketched matrices as noted in \cref{sec:sd}.
\end{remark}

\subsection{Inexact sub-solvers for practical usage}
In practice, the \ff{M-IHS} and \ff{Dual M-IHS} eliminate the dominant term $O(md^2)$ in the complexity expression of moderns solver such as the Blendenpik and LSRN by approximately solving the low dimensional linear systems in \cref{eq:mihs1} and \cref{eq:dual_mihs1} instead of computing a matrix decomposition or an inversion. This \textit{inexact sub-solver} approach constitutes a trade-off between the computational complexity and the accuracy, that is highly desirable in very large dimensional problems where solutions with relatively lower accuracy are acceptable. Unfortunately, forming this trade-off is not possible for the Blendenpik and LSRN techniques which require a full matrix decomposition. Inexact sub-solvers have been known to be a good heuristic way to create this trade-off and they are widely used in the algorithms that are based on the Newton Method to solve the large scale normal equations \cite{ref:nocedal}. In these inexact (or truncated) Newton Methods, inner iterations are terminated at the moment that the relative residual error is below some iteration dependent threshold, named as the \textit{forcing terms} \cite{ref:forcing_term}. In the literature, there are various techniques to choose these forcing terms that guarantee global convergence, but the number of iterations suggested by these techniques are far above the total number of iterations used in practice. We refer interested reader to \cite{ref:inexact_survey} and we go forward with the heuristic constant threshold, $\epsilon_{sub}$, that checks the relative residual error of the linear system \cite{ref:nocedal2}.

Any Krylov subspace based first order method can be used to (inexactly) solve the sub-problems in \cref{eq:mihs1} and \cref{eq:dual_mihs1}, but LSQR-like solvers that are adapted for the normal equations would require computations of 4 matrix-vector multiplications per iteration. On the other hand, due to the explicit calculation of $(SA)^T(SA)z$, the symmetric CG, that would require only 2 matrix-vector multiplications, might be unstable in the ill-conditioned problems \cite{ref:lsqr}. Therefore, in \cref{sec:subsolver}, we propose a stable sub-solver which is particularly designed for the problems in the form of $A^TAx=b$. The proposed sub-solver, referred to as \ff{AAb\_Solver}, is based on the Golub Kahan Bidiagonalization and it uses a similar approach that the LSQR uses on the LS problem. In addition to the stability advantage over symmetric CG technique, \ff{AAb\_Solver} produces a bidiagonal representation of sketched matrix as a byproduct of the iterations. This bidiagonal form can be used in, for example, Generalized Cross Validation \cite{ref:gcv, ref:siam_review_hybrid} to estimate the problem related parameters including the regularization parameter and the statistical dimension. The inexact versions of the \ff{M-IHS} and \ff{Dual M-IHS} that use \ff{AAb\_Solver} are given in \cref{algo:mihs} and \cref{algo:dual_mihs} where \ff{RP\_fun} represents the function that generates the desired sketched matrix such that $\expectt{}{S^TS} = I_m$ whose implementation details can be found in the relevant references in \cref{corollary:sketch}. Number of operations required at each line is stated at the right most column of the algorithms. $C(\cdot)$ represents the complexity of constructing the sketching matrix as given in \cref{corollary:sketch}. %%%
\subfile{demos/algo_mihs.tex}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Setting the forcing term $\epsilon_{sub}$, for instance, to 0.5 for all iterations is enough for the inexact \ff{M-IHS} variants to converge at the same rate $\sqrt{\beta}$ as the exact versions as demonstrated in \cref{fig:convergence}.

\Cref{corollary:sketch} suggests that if the statistical dimension is several times smaller than the dimensions of $A$, then it is possible to choose a substantially smaller sketch size than $\min(n,d)$. If this is the case, then the quadratic objective functions in \cref{eq:mihs1} and \cref{eq:dual_mihs1} become strongly under-determined problems, which makes it possible to approximate the Hessian of the objective functions one more time by taking their convex dual as it has been done in the \ff{Dual M-IHS}. This approach is similar to approximately solving the problems in \cref{eq:mihs1} and \cref{eq:dual_mihs1} by using the \ff{AAb\_Solver}, but this time we are going to apply a second dimension reduction. At the end of two Hessian sketching, the linear sub-problem whose dimensions are reduced from both sides can be efficiently solved by the \ff{AAb\_Solver} for a pre-determined tolerance as before. Consider the following dual of the sub-problem in \cref{eq:mihs1}
\begin{equation}
    z^* = \swrite{argmin }{z\in\reals{m}} \underbrace{\frac{1}{2}\lscost{A^TS^Tz + \nabla f(x^i)}{2}^2 + \frac{\lambda}{2}\lscost{z}{2}^2}_{h(x^i,z)},
\end{equation}
which is a strongly over-determined problem if $m\ll \min(n,d)$. Hence, it can be approximately solved by the \ff{M-IHS} updates as
\begin{align}
    \Delta z^j &= \swrite{argmin }{z\in\reals{m}} \lscost{WA^TS^Tz}{2}^2 + \lambda\lscost{z}{2}^2 + 2\left\langle \nabla_z h(x^i, z^j), \ z\right\rangle \label{eq:pd_mihs1},\\
    z^{j+1}&= z^j + \alpha_2\Delta z^j + \beta_2 \left(z^j - z^{j-1}\right). \nonumber
\end{align}
After $M$ iterations, the solution of \cref{eq:mihs1} can be recovered by using the relation in \cref{eq:dual_relation} as $\Delta x^i = (\nabla f(x^i) - A^TS^Tz^M)/\lambda$. The same strategy can be applied on the sub-problem in \cref{eq:dual_mihs1} by replacing $SA$ with $SA^T$ and $\nabla f(x^i)$ with $\nabla g(\nu^i)$. The resulting algorithms, referred to as \ff{Primal Dual M-IHS}, are given in \cref{algo:pd_mihs_1} and \cref{algo:pd_mihs_2} respectively.%
\subfile{demos/algo_pd.tex}

The primal-dual idea presented here is first suggested by Zhang et al. in \cite{ref:acc_ihs}. They used the A-IHS technique to solve the sub-problems that arise during the iterations of the Accelerated Iterative Dual Random Projection (A-IDRP) which is a dual version of the A-IHS. However, since both of the A-IHS and the A-IDRP are based on the CG technique, the convergence rate of the proposed A-IHS, A-IDRP and the primal dual algorithm called as Accelerated Primal Dual Sketch (A-IPDS) are all degraded in the LS problems with high condition numbers due to the instability issue of the symmetric CG technique \cite{ref:lsqr}. Even if the regularization is used, still the performance of the solvers proposed in \cite{ref:acc_ihs} are considerably deteriorated compared to the other randomized preconditioning techniques as shown in \cref{sec:numeric}. Further, applying the preconditioning idea of IHS to the stable techniques such as the LSQR that are adapted for the LS problem is not so efficient as the \ff{M-IHS} variants, because then two preconditioning systems are needed to be solved per iteration for such techniques.

The computational saving when we apply a second dimension reduction as in the \ff{Primal Dual M-IHS} may not be significant due to the second gradient computations in Line 10 and 9 of the given algorithms, but the lower dimensional sub-problems that we obtain at the end of the second sketching can be used to estimate several parameters including the regularization parameter itself. Indeed, we are currently working on such an algorithm to estimate the regularization parameter of the large scale problems along with the iterations of the \ff{M-IHS} variants without requiring additional accesses to coefficient matrix $A$ except for the computation of the gradients. 

The \ff{Primal Dual M-IHS} techniques are extension of the inexact schemes. Therefore, their convergence rates depend on their forcing terms that are used to stop the inner iterations \cite{ref:inexact_survey}. In \cite{ref:acc_ihs}, an upper bound for the error of the primal dual updates is proposed. However as it is detailed in \cref{sec:app}, there are several inaccuracies in the development of the bound. Therefore, finding a provably valid lower bound on the number of inner loop iterations, that guarantee a certain rate of convergence at the main loop, is still an open question for the primal dual algorithms.

==> sections/theory.tex <==
In this section, we are going to provide a unified analysis of the regularized LS problems through the proofs by including many comments and explanations. Throughout the analysis we denote $A = U\Sigma V^T$ as the compact SVD with $U\in\realss{n}{r}$, $\Sigma = \diag(\sigma_1,\ldots,r)\in\realss{r}{r}$ and $V \in\realss{d}{r}$ where $r =\min(n,d)$.

\subsection{Proof of \Cref{lemma:mihs_conv}} \label{proof:lemma_conv}
To prove the theorem for the \ff{M-IHS} and the \ff{Dual M-IHS}, we mainly combine the idea of \textit{partly exact} sketching, that is proposed in \cite{ref:acw16_sharper}, with the Lyapunov analysis, that we use in \cite{ref:mihs}. In parallel to \cite{ref:acw16_sharper}, we define diagonal matrix $D:=(\Sigma^2 + \lambda I_{r})^{-1/2}$ and the \textit{partly exact} sketching matrix as:
\begin{equation*}
    \widehat{S} = \begin{bmatrix}S &\mathbf{0}\\\mathbf{0} & I_r\end{bmatrix}, \quad S\in\realss{m}{\max(n,d)}.
\end{equation*}
\paragraph{The Proof for M-IHS:} 
Let
\begin{equation*}
    \widehat{A} = \begin{bmatrix} U\Sigma D \\ \sqrt{\lambda} VD\end{bmatrix} = \begin{bmatrix} U_1 \\U_2\end{bmatrix}, \quad \widehat{A}^T\widehat{A} = I_d, \quad \widehat{b} = \begin{bmatrix}b\\\mathbf{0}\end{bmatrix},
\end{equation*}
so that $U_1$ is the first $n$ rows of an orthogonal basis for $\begin{bmatrix}A\\ \sqrt{\lambda} I_d \end{bmatrix}$ as required by the condition in \cref{condition:1} of the theorem. We have the following equality
\begin{equation*}
    \lscost{Ax - b}{2}^2 +\lambda\lscost{x}{2}^2 = \lscost{\widehat{A}y - \widehat{b}}{2}^2, \mbox{ for } \left\{\forall x \in\reals{d}\ |\ y = D^{-1}V^Tx \right\},
\end{equation*}
and the sketched matrix
\begin{equation*}
     \quad \widehat{S}\widehat{A} = \begin{bmatrix} SU\Sigma D\\ \sqrt{\lambda}VD\end{bmatrix} = \begin{bmatrix} SU_1\\U_2\end{bmatrix}.
\end{equation*}
Since the following Hessian Sketch (HS) sub-problem
\begin{equation*}
    \Delta y^{i} = \swrite{argmin}{y} \lscost{\widehat{S}\widehat{A}y}{2}^2 - 2\langle \widehat{A}^T(\widehat{b} - \widehat{A}y^i), \ y \rangle
\end{equation*}
is equivalent to \cref{eq:mihs1}, we can examine the following bipartite transformation to find out the convergence properties of the \ff{M-IHS}:
\begin{equation*}
    \begin{bmatrix}
    y^{i+1} - y^* \\
    y^{i} - y^*
    \end{bmatrix} = \underbrace{\begin{bmatrix}
    (1+\beta)I_d - \alpha (\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A})^{-1} & -\beta I_d\\
    I_d & \mathbf{0}
    \end{bmatrix}}_{T} \begin{bmatrix}
    y^{i} - y^* \\
    y^{i-1} - y^*
    \end{bmatrix},
\end{equation*}
where $y^* = D^{-1}V^Tx^*$ and $\widehat{A}^T\widehat{A} = I_d$. The eigenvalues and therefore the contraction ratio of the transformation can be found analytically by converting the matrix $T$ into a block diagonal form through the same similarity transformation given in \cite{ref:mihs}:
\begin{align*}
T &= P^{-1} \diag(T_1,\ldots, T_d) P,\quad T_i := \begin{bmatrix}
    1 + \beta - \alpha \lambda_i & \beta \\
    1 & 0
\end{bmatrix}, \\
P &= \begin{bmatrix}
    \Psi & 0 \\
    0 & \Psi
\end{bmatrix} \Pi, \quad\quad\qquad\qquad
\Pi_{i,j} = \left\{
\small\begin{array}{rl}
1 & \text{i \mbox{is odd} } j = i,\\
1 &  \text{i \mbox{is even} } j = r+i,\\
0 &  \text{otherwise,}
\end{array} \right.
\end{align*}
where $\Psi \Lambda \Psi^T$ is the Spectral decomposition of $(\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A})^{-1}$ and $\lambda_i$ is the $i^{th}$ eigenvalue. The characteristic polynomials of each block is
\begin{equation*}
    u^2 - (1+\beta - \alpha \lambda_i)u + \beta = 0, \quad \forall i \in [r].
\end{equation*}
If the following condition holds
\begin{equation}
    \beta \geq (1 - \sqrt{\alpha \lambda_i})^2, \quad \forall i \in [r] \label{condition:dynamic},
\end{equation}
then both of the roots are imaginary and both have a magnitude $\sqrt{\beta}$ for all $\lambda$'s. In this case, all linear dynamical systems driven by above characteristic polynomial will be in the under-damped regime and the contraction rate of the transformation $T$, through all directions, not just one of them, will be exactly $\sqrt{\beta}$. If the condition in \cref{condition:dynamic} is not satisfied for a $\lambda_j$ with $j\in [r]$, then the linear dynamical system corresponding to $\lambda_j$ will be in the over-damped regime and the contraction rate in the direction through the eigenvector corresponding to this over-damped system will be smaller compared to the others. As a result, the overall algorithm will be slowed down substantially (see \cite{ref:candes_adaptive} for details). If the condition in \cref{condition:1} of \cref{lemma:mihs_conv} holds,
\begin{equation*}
    \lscost{\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A} - I_r}{2} = \lscost{U_1^TS^TSU_1 +U_2^TU_2- I_r}{2}=\lscost{U_1^TS^TSU_1 - U_1^TU_1}{2}\leq \epsilon,
\end{equation*}
then
\begin{equation*}
    \swrite{sup }{\lscost{v}{2} = 1}v^T\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}v \leq 1+\epsilon \quad\mbox{   and   }\quad \swrite{inf }{\lscost{v}{2} = 1}v^T\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}v \geq 1-\epsilon,
\end{equation*}
and
\begin{equation*}
    \swrite{maximize}{ i \in [r]} \lambda_i \leq \frac{1}{1-\epsilon} \quad \mbox{   and   }\quad \swrite{minimize}{ i \in [r]} \lambda_i \geq \frac{1}{1+\epsilon}.
\end{equation*}
Consequently, the condition in \cref{condition:dynamic} can be satisfied for all $\lambda_i$'s by the following choice of $\beta$ that maximizes the convergence rate over step size $\alpha$
\begin{equation*}
    \sqrt{\beta^*} = \swrite{minimize}{\alpha}\!\left(\max\left\{1 - \frac{\sqrt{\alpha}}{\sqrt{1 +\epsilon}},\ \frac{\sqrt{\alpha}}{\sqrt{1 - \epsilon}} - 1 \right\}\right) =  \frac{\epsilon}{1 + \sqrt{1 -\epsilon^2}},
\end{equation*}
where the minimum is achieved at $\alpha^* = \frac{4(1 - \epsilon^2)}{(\sqrt{1+\epsilon}+\sqrt{1 - \epsilon})^2} = (1- \beta^*)\sqrt{1 - \epsilon^2}$ as claimed.

\paragraph{The Proof for Dual M-IHS:}
The proof for the dual counter-part is almost same as the proof for \ff{M-IHS} except for the following modifications. Let
\begin{equation*}
    \widehat{A}^T = \begin{bmatrix} V\Sigma D \\ \sqrt{\lambda} UD\end{bmatrix}=\begin{bmatrix} U_1\\U_2\end{bmatrix}, \ \widehat{A}\widehat{A}^T = I_n \ \mbox{ and }\ \widehat{S}\widehat{A}^T = \begin{bmatrix} SV\Sigma D\\ \sqrt{\lambda}UD\end{bmatrix} = \begin{bmatrix} SU_1\\U_2\end{bmatrix},
\end{equation*}
so that $U_1$ is the first $d$ rows of an orthogonal basis for $\begin{bmatrix}A^T\\ \sqrt{\lambda} I_n \end{bmatrix}$ as required by the theorem. We have the following equality:
\begin{equation*}
    \frac{1}{2}\lscost{A^T\nu}{2}^2 + \frac{1}{2}\lscost{\nu}{2}^2 - \langle b,\ \nu \rangle = \frac{1}{2}\lscost{\widehat{A}^Tw}{2}^2 - \langle DU^Tb,\ w\rangle,
\end{equation*}
for $\left\{\forall \nu \in\reals{n}\ |\ w = D^{-1}U^T\nu \right\}$. Thus, following HS sub-problem is equivalent to \cref{eq:dual_mihs1}
\begin{equation*}
    \Delta w^{i+1} = \swrite{argmin}{y} \lscost{\widehat{S}\widehat{A}^Tw}{2}^2 - 2\langle DU^Tb -  \widehat{A}\widehat{A}^Tw^i, \ w \rangle.
\end{equation*}
We can analyze the following bipartite transformation to figure out the convergence properties of the \ff{Dual M-IHS}
\begin{equation*}
    \begin{bmatrix}
    w^{i+1} - w^* \\
    w^{i} - w^*
    \end{bmatrix} = \underbrace{\begin{bmatrix}
    (1+\beta)I_n - \alpha (\widehat{A}\widehat{S}^T\widehat{S}\widehat{A}^T)^{-1} & -\beta I_n\\
    I_n & \mathbf{0}
    \end{bmatrix}}_{T} \begin{bmatrix}
    w^{i} - w^* \\
    w^{i-1} - w^*
    \end{bmatrix},
\end{equation*}
where $w^* = D^{-1}U^Tv^*$. The rest of the proof can be completed straightforwardly by following the same analysis steps as in the proof for the \ff{M-IHS} case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of the Condition in \cref{lemma:mihs_conv}}\label{proof:cor_sketch}
\Cref{lemma:mihs_conv} is valid if the sketch matrix $S$ satisfies the following condition:
\begin{equation}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2} \leq \lscost{U_1^TS^TSU_1 - U_1^TU_1}{F} \leq \epsilon, \label{eq:aim}
\end{equation}
where
\begin{equation*}
    \lscost{U_1}{F}^2 = \lscost{U\Sigma D}{F}^2 = \lscost{\Sigma(\Sigma^2 +\lambda I_r)^{-1/2}}{F}^2 = \sum\limits_{i=1}^{r}\frac{\sigma_i^2}{\sigma_i^2 + \lambda} = \sd(A),
\end{equation*}
and $\lscost{U_1}{2}^2 = \frac{\sigma_1^2}{\sigma_1^2 + \lambda} \approx 1$ for a properly chosen regularization parameter $\lambda$. In this subsection before giving the proof of \cref{corollary:sketch}, we summarize some of the current results and tools from the random matrix theory literature that is used to prove the condition in \cref{eq:aim} for different applications such as low rank approximation, matrix ridge regression, kernel ridge regression, $\ell_p$ regression, k-means clustering.

If the sketch matrix $S$ is drawn from a randomized distribution $\D$ over matrices $\realss{m}{n}$, then the condition in \cref{eq:aim} can be met with a desired level of probability. 
\begin{definition} (JL Lemma \cite{ref:jl_lemma}) \label{def:jl_distribution} For any integer $n>0$, $\epsilon, \delta< 1/2$, the distribution $\D$ over $S\in\realss{m}{n}$ is called as $(\epsilon, \delta)-$JL distribution if for any $x\in\reals{n}$,
\begin{equation*}
    \prob{S\sim \D}{(1-\epsilon)\lscost{x}{2}\leq\lscost{Sx}{2} \leq (1+\epsilon)\lscost{x}{2}} > 1-\delta,
\end{equation*}
holds for $m = \Theta(\epsilon^{-2}\log(1/\delta))$.
\end{definition}
The sketch size given in the definition is optimal \cite{ref:kn14_sparser_jl}. By assuming $x$ is unit norm, the probability in \cref{def:jl_distribution} can be bounded by the Markov Inequality \cite{ref:w14_sketching_asatool, ref:nn13_osnap}:
\begin{align*}
    \prob{S\sim \D}{\big|\lscost{Sx}{2}-1\big|> \epsilon} &= \prob{S\sim \D}{\big|\lscost{Sx}{2}-1\big|^\ell> \epsilon} \\
    &\leq \epsilon^{-\ell}\cdot\expectt{S\sim \D}{\big|\lscost{Sx}{2}-1\big|^\ell},
\end{align*}
which leads to a fundamental property:
\begin{definition}\label{def:jl_moment}(JL-Moment Property Definition 6.1 in \cite{ref:kn14_sparser_jl}) Distribution $\D$ over $\realss{m}{n}$ has $(\epsilon,\delta,\ell)$-JL moment property if for all the unit norm vectors $x\in\reals{n}$
\begin{equation*}
    \expectt{S\sim\D}{|\lscost{Sx}{2}^2-1|^\ell} \leq \epsilon^\ell\cdot\delta.
\end{equation*}
\end{definition}
Having JL-moment property is a stronger condition than being a JL-distribution, but if a distribution $\D$ is a $(\epsilon, e^{-\Omega(\epsilon^2m)})$-JL distribution, then it is called as \textit{Strong JL Distribution} \cite{ref:kmn_11_almost_optimal} and it automatically verifies the $(\epsilon, e^{-\Omega(\epsilon^2m)}, \min(\epsilon^2m,\ \epsilon m))$-JL moment property \cite{ref:kn14_sparser_jl}. The JL-moment property is important to reach our goal due to the following property called the Approximate Matrix Multiplication (AMM):
\begin{theorem}\label{theorem:kn_amm} (AMM Property, Theorem 6.2 in \cite{ref:kn14_sparser_jl})
Given $\epsilon, \delta\in(0,1/2)$, let $\D$ be any distribution over matrices in $\realss{m}{n}$ with the $(\epsilon, \delta,\ell)$-JL moment property for some $\ell\geq 2$. Then for any $A,B\in\realss{n}{d}$ real matrices,
\begin{equation*}
    \prob{S\sim\D}{\lscost{A^TS^TSB - A^TB}{F}<3\epsilon\lscost{A}{F}\lscost{B}{F}} > 1- \delta.
\end{equation*}
\end{theorem}
If the sketch matrix satisfies the JL-moment property, setting $A=B=U_1$ in the AMM property gives the condition in \ref{eq:aim}, but except for the sparse sketch matrices with single non-zero element in each column, the AMM property that is based on the JL-Distribution is too restrictive for the other sketch types mentioned in \cref{corollary:sketch} to satisfy the condition. For them, the $\ell2$ subspace embeddings, which is introduced in \cite{ref:sar06_l2_embedding}, can be used.

\begin{definition}\label{def:osa}(Oblivious $\ell2$ Subspace Embedding (OSE)) If a distribution $\D$ satisfies
$$
    \prob{S\sim\D}{\lscost{US^TSU - I}{2} >\epsilon} <\delta,
$$
with $U\in\realss{n}{k}, \ U^TU = I_k, \ S\in\realss{m}{n}$, then it is called $(\epsilon, \delta, k)$-OSE.
\end{definition}
The JL-distributions are special case of $(\epsilon,\delta,k)$-OSE with $k = n$. While the JL distributions projects the whole $\reals{n}$, the OSE distributions embed only a subspace \textbf{span}$(U)\subseteq\reals{n}$. Consequently, the subspace embeddings provide a more general moment property.
\begin{definition}\label{def:ose_moment}(OSE Moment Property \cite{ref:cnw15_optimal_stable_rank}) A distribution $\D$ over $S\in\realss{m}{n}$ has $(\epsilon, \delta, k,\ell)$-OSE Moment Property, if for all matrices $U\in\realss{n}{k}$ with orthonormal columns,
$$
\expectt{S\sim\D}{\lscost{U^TS^TSU - I_k}{2}^\ell} < \epsilon^{-\ell}\cdot\delta.
$$
\end{definition}
The JL moment property is the special case of the OSE moment property with $k = n$ and the relation between them is given in the following lemma.
\begin{lemma}\label{lemma:jl_ose_cnw15}(Lemma 4 of \cite{ref:cnw15_optimal_stable_rank}) If a distribution $\D$ satisfies the $(\epsilon, \delta,\ell)$-JL moment property, then $\D$ satisfies the $(2\epsilon, 9^k\delta, k,\ell)$-OSE moment property.
\end{lemma}
By using the OSE Moment property to obtain a generalized AMM property is also possible:
\begin{theorem}\label{theorem:amm_ose}($(\epsilon, \delta, k)$-AMM Property \cite{ref:cnw15_optimal_stable_rank}) If a distribution $\D$ over $S\in\realss{m}{n}$ has the $(\epsilon, \delta, 2k,\ell)$-OSE moment property for some $\delta <1/2$ and $\ell\geq2$, then for any $A,B$:
$$
\prob{S\sim\D}{\lscost{A^TS^TSB - A^TB}{2} > \epsilon\sqrt{\left(\lscost{A}{2}^2+ \frac{\lscost{A}{F}^2}{k}\right)\left(\lscost{B}{2}^2 + \frac{\lscost{B}{F}^2}{k}\right)}} < \delta.
$$
\end{theorem}
\Cref{theorem:amm_ose} breaks the dependence between the error constant $\epsilon$ and the sketch size $m$ in the AMM property given in \cref{theorem:kn_amm}. By \cref{theorem:amm_ose}, the sketch sizes can be chosen in accordance with the embedding size $k$ to satisfy the condition in \cref{eq:aim} as we will show next.

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item1}} Count Sketch with a single nonzero element in each column and size $m\geq 2/({\epsilon'}^2\delta)$ has $(\epsilon', \delta,2)$-JL moment property \cite{ref:tz12}. By \cref{theorem:kn_amm}:
\begin{equation*}
    \lscost{U_1S^TSU_1 - U_1^TU_1}{F} < 3\epsilon'\lscost{U_1}{F}^2 = 3\epsilon'\sd(A) \leq \epsilon
\end{equation*}
for $\epsilon' = \epsilon/(3\sd(A))$. So, condition in \cref{eq:aim} holds with probability at least $1-\delta$, if $m = O(\sd(A)^2/(\epsilon^2\delta))$. 

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item2}} Combining Theorem 4.2 of \cite{ref:coh16_nearly_tight} and Remark 2 of \cite{ref:cnw15_optimal_stable_rank} implies that any sketch matrix drawn from an OSNAP \cite{ref:nn13_osnap} with the conditions given in the item $(ii)$ of \cref{corollary:sketch} satisfies the $(\epsilon', \delta, k, \log(k/\delta))$-OSE moment property, thus the $(\epsilon', \delta, k/2)$-AMM Property. Setting $A=B=U_1$  and $k = \sd(A)/2$ in \cref{theorem:amm_ose} gives:
\begin{equation*}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2} \leq \epsilon'(\lscost{U_1}{2}^2 + 2) \leq 3 \epsilon' \leq \epsilon
\end{equation*}
with probability at least $1-\delta$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}
Based on the lower bounds established for any OSE in \cite{ref:nn14_lower}, the Conjecture 14 in \cite{ref:nn13_osnap} states that any OSNAP with 
$m=\Omega((k+\log(1/\delta))/\epsilon^2)$ and 
$s=\Omega(\log(k/\delta)/\epsilon)$ have the $(\epsilon,\delta,k,\ell)$-OSE moment property for $\ell = \Theta(\log(k/\delta))$, an even integer. As a result of the conjecture and \cref{theorem:amm_ose}, the condition in \cref{eq:aim} can be satisfied with probability at least $1-\delta$ by using an OSNAP matrix with size $m=\Omega((\sd(A)+\log(1/\delta))/\epsilon^2)$ and sparsity $s=\Omega(\log(\sd(A)/\delta)/\epsilon)$.
\end{remark}
\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item3}} By Theorem 9 of \cite{ref:cnw15_optimal_stable_rank}, SRHT with the sketch size given in item $(iii)$ has the $(\epsilon', \delta, 2\sd(A), \log(\sd(A)/\delta))$-OSE moment property and thus by \cref{theorem:amm_ose}, it provides $(\epsilon', \delta, \sd(A))$-AMM property. Again, setting $A=B=U_1$ and $k=\sd(A)$ produces the desired result.

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item4}} The Subgaussian matrices having entries with mean zero and variance $1/m$ satisfy the \cref{def:jl_distribution} with optimal sketch size. Also, they have the $(\epsilon/2, \delta, \Theta(\log(1/\delta)))$-JL moment property \cite{ref:kmn_11_almost_optimal}. Thus by \cref{lemma:jl_ose_cnw15} such matrices have $(\epsilon,\delta,k,\Theta(k+\log(1/\delta)))$-OSE moment property for $\delta < 9^{-k}$, which means $m=\Omega(k/\epsilon^2)$. Again, by setting $A=B=U_1$ and $k = \sd(A)$ in \cref{theorem:amm_ose} gives the desired result.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence proof without regularization} \label{proof:no_reg}
If the LS problem without any regularization is tried to be solved, then we need the following inequality to hold:
\begin{equation*}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2}\leq \epsilon \xRightarrow[n\geq d]{\quad\lambda\to0\quad }\lscost{U^TS^TSU - I_r}{2}\leq \epsilon,
\end{equation*}
which can be satisfied with a constant probability, if the sketch matrix is drawn from a distribution $\D$ that has the OSE Moment property defined in \cref{def:ose_moment}. Then, the bound for the sketch size can be derived by using the other results presented above. The details of how to obtain the above inequality can be found in \cite{ref:mihs}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of \cref{corollary:empirical}} \label{proof:empirical}
Consider the regularized LS solution with parameter $\lambda$ and the Truncated SVD solution with parameter $\lceil\sd(A)\rceil$:
\begin{equation*}
    x^* = \sum\limits_{i=1}^r \frac{\sigma_i^2}{\sigma_i^2 + \lambda}\frac{u_i^Tb}{\sigma_i}v_i \quad\mbox{ and }\quad x^\dagger = \sum\limits_{i=1}^{\lceil\sd(A)\rceil}\frac{u_i^Tb}{\sigma_i}v_i
\end{equation*}
where $u_i$'s and $v_i$'s are columns of $U$ and $V$ matrices in the SVD. The Tikhonov regularization with the closed form solution is preferred in practise to avoid the high computational cost of the SVD. The filtering coefficients of the Tikhonov regularization, $\frac{\sigma_i^2}{\sigma_i^2 + \lambda}$, become very close to the binary filtering coefficients of the TSVD, as the decay rate of the singular values of $A$ increases. In these cases, both the solution $x^*$ and $x^\dagger$ become almost indistinguishable. Thereby, the diagonal matrix, $\Sigma D$, which is used in the proof of \cref{corollary:sketch} can be approximated by the diagonal matrix $\Pi$ where
\begin{equation*}
    \Pi_{ii} = \left\{
\begin{array}{rl}
1 & \text{if } i \leq \sd(A) \leq r\\
0 &  otherwise
\end{array} \right.,
\end{equation*}
which is equivalent to replace the Tikhonov coefficients by the binary TSVD coefficients. Then, we have
\begin{align*}
    \left(\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}\right)^{-1} &= \left(D\Sigma U^TS^TSU\Sigma D + \lambda D^2\right)^{-1}\\ &\approx \left(\Pi (SU)^T(SU)\Pi + I_r - \Pi\right)^{-1} = \left[\begin{array}{c|c}
        \widebar{S}^T\widebar{S}& \textbf{0}\\
        \hline
        \textbf{0} & I_{(r - \sd(A))}
    \end{array}\right],
\end{align*}
where $\widebar{S} = SU\Pi\in\realss{m}{\sd(A)}$ has the same distribution as $S$, since $U\Pi$ is an orthonormal transformation. By the Marchenko Pastur Law, the minimum and the maximum eigenvalues of this approximation converge to $\left(1 \pm \sqrt{\frac{\sd(A)}{m}}\right)^{-2}$ as $m\to \infty$ and while $\sd(A)/m$ remains constant \cite{ref:edelman2, ref:edelman}. The rest of the proof follows from the analysis given in \cref{proof:lemma_conv}.

==> sections/theory_short.tex <==
In this section, we are going to provide proofs of the theoretical claims given in the main text. We will use a unified analysis for both under-determined and over-determined problems. Throughout the analysis we denote $A = U\Sigma V^T$ as the compact SVD with $U\in\realss{n}{r}$, $\Sigma = \diag(\sigma_1,\ldots,r)\in\realss{r}{r}$ and $V \in\realss{d}{r}$ where $r =\min(n,d)$.

\subsection{Proof of \Cref{lemma:mihs_conv}} \label{proof:lemma_conv}
To prove the theorem for the \ff{M-IHS} and the \ff{Dual M-IHS}, we mainly combine the idea of \textit{partly exact} sketching, that is proposed in \cite{ref:acw16_sharper}, with the Lyapunov analysis, that we use in \cite{ref:mihs}. In parallel to \cite{ref:acw16_sharper}, we define diagonal matrix $D:=(\Sigma^2 + \lambda I_{r})^{-1/2}$ and the \textit{partly exact} sketching matrix as:
\begin{equation*}
    \widehat{S} = \begin{bmatrix}S &\mathbf{0}\\\mathbf{0} & I_r\end{bmatrix}, \quad S\in\realss{m}{\max(n,d)}.
\end{equation*}
\paragraph{The Proof for M-IHS:} 
Let
\begin{equation*}
    \widehat{A} = \begin{bmatrix} U\Sigma D \\ \sqrt{\lambda} VD\end{bmatrix} = \begin{bmatrix} U_1 \\U_2\end{bmatrix}, \quad \widehat{A}^T\widehat{A} = I_d, \quad \widehat{b} = \begin{bmatrix}b\\\mathbf{0}\end{bmatrix},
\end{equation*}
so that $U_1$ is the first $n$ rows of an orthogonal basis for $\begin{bmatrix}A\\ \sqrt{\lambda} I_d \end{bmatrix}$ as required by the condition in \cref{condition:1} of the theorem. We have the following equality
\begin{equation*}
    \lscost{Ax - b}{2}^2 +\lambda\lscost{x}{2}^2 = \lscost{\widehat{A}y - \widehat{b}}{2}^2, \mbox{ for } \left\{\forall x \in\reals{d}\ |\ y = D^{-1}V^Tx \right\},
\end{equation*}
and the sketched matrix
\begin{equation*}
     \quad \widehat{S}\widehat{A} = \begin{bmatrix} SU\Sigma D\\ \sqrt{\lambda}VD\end{bmatrix} = \begin{bmatrix} SU_1\\U_2\end{bmatrix}.
\end{equation*}
Since the following Hessian Sketch (HS) sub-problem
\begin{equation*}
    \Delta y^{i} = \swrite{argmin}{y} \lscost{\widehat{S}\widehat{A}y}{2}^2 - 2\langle \widehat{A}^T(\widehat{b} - \widehat{A}y^i), \ y \rangle
\end{equation*}
is equivalent to \cref{eq:mihs1}, we can examine the following bipartite transformation to find out the convergence properties of the \ff{M-IHS}:
\begin{equation*}
    \begin{bmatrix}
    y^{i+1} - y^* \\
    y^{i} - y^*
    \end{bmatrix} = \underbrace{\begin{bmatrix}
    (1+\beta)I_d - \alpha (\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A})^{-1} & -\beta I_d\\
    I_d & \mathbf{0}
    \end{bmatrix}}_{T} \begin{bmatrix}
    y^{i} - y^* \\
    y^{i-1} - y^*
    \end{bmatrix},
\end{equation*}
where $y^* = D^{-1}V^Tx^*$ and $\widehat{A}^T\widehat{A} = I_d$. The eigenvalues and therefore the contraction ratio of the transformation can be found analytically by converting the matrix $T$ into a block diagonal form through the same similarity transformation given in \cite{ref:mihs}:
\begin{align*}
T &= P^{-1} \diag(T_1,\ldots, T_d) P,\quad T_i := \begin{bmatrix}
    1 + \beta - \alpha \lambda_i & \beta \\
    1 & 0
\end{bmatrix}, \\
P &= \begin{bmatrix}
    \Psi & 0 \\
    0 & \Psi
\end{bmatrix} \Pi, \quad\quad\qquad\qquad
\Pi_{i,j} = \left\{
\small\begin{array}{rl}
1 & \text{i \mbox{is odd} } j = i,\\
1 &  \text{i \mbox{is even} } j = r+i,\\
0 &  \text{otherwise,}
\end{array} \right.
\end{align*}
where $\Psi \Lambda \Psi^T$ is the Spectral decomposition of $(\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A})^{-1}$ and $\lambda_i$ is the $i^{th}$ eigenvalue. The characteristic polynomials of each block is
\begin{equation*}
    u^2 - (1+\beta - \alpha \lambda_i)u + \beta = 0, \quad \forall i \in [r].
\end{equation*}
If the following condition holds
\begin{equation}
    \beta \geq (1 - \sqrt{\alpha \lambda_i})^2, \quad \forall i \in [r] \label{condition:dynamic},
\end{equation}
then both of the roots are imaginary and both have a magnitude $\sqrt{\beta}$ for all $\lambda$'s. In this case, all linear dynamical systems driven by above characteristic polynomial will be in the under-damped regime and the contraction rate of the transformation $T$, through all directions, not just one of them, will be exactly $\sqrt{\beta}$. If the condition in \cref{condition:dynamic} is not satisfied for a $\lambda_j$ with $j\in [r]$, then the linear dynamical system corresponding to $\lambda_j$ will be in the over-damped regime and the contraction rate in the direction through the eigenvector corresponding to this over-damped system will be smaller compared to the others. As a result, the overall algorithm will be slowed down substantially (see \cite{ref:candes_adaptive} for details). If the condition in \cref{condition:1} of \cref{lemma:mihs_conv} holds,
\begin{equation*}
    \lscost{\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A} - I_r}{2} = \lscost{U_1^TS^TSU_1 +U_2^TU_2- I_r}{2}=\lscost{U_1^TS^TSU_1 - U_1^TU_1}{2}\leq \epsilon,
\end{equation*}
then
\begin{equation*}
    \swrite{sup }{\lscost{v}{2} = 1}v^T\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}v \leq 1+\epsilon \quad\mbox{   and   }\quad \swrite{inf }{\lscost{v}{2} = 1}v^T\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}v \geq 1-\epsilon,
\end{equation*}
and
\begin{equation*}
    \swrite{maximize}{ i \in [r]} \lambda_i \leq \frac{1}{1-\epsilon} \quad \mbox{   and   }\quad \swrite{minimize}{ i \in [r]} \lambda_i \geq \frac{1}{1+\epsilon}.
\end{equation*}
Consequently, the condition in \cref{condition:dynamic} can be satisfied for all $\lambda_i$'s by the following choice of $\beta$ that maximizes the convergence rate over step size $\alpha$
\begin{equation*}
    \sqrt{\beta^*} = \swrite{minimize}{\alpha}\!\left(\max\left\{1 - \frac{\sqrt{\alpha}}{\sqrt{1 +\epsilon}},\ \frac{\sqrt{\alpha}}{\sqrt{1 - \epsilon}} - 1 \right\}\right) =  \frac{\epsilon}{1 + \sqrt{1 -\epsilon^2}},
\end{equation*}
where the minimum is achieved at $\alpha^* = \frac{4(1 - \epsilon^2)}{(\sqrt{1+\epsilon}+\sqrt{1 - \epsilon})^2} = (1- \beta^*)\sqrt{1 - \epsilon^2}$ as claimed.

\paragraph{The Proof for Dual M-IHS:}
The proof for the dual counter-part is almost same as the proof for \ff{M-IHS} except for the following modifications. Let
\begin{equation*}
    \widehat{A}^T = \begin{bmatrix} V\Sigma D \\ \sqrt{\lambda} UD\end{bmatrix}=\begin{bmatrix} U_1\\U_2\end{bmatrix}, \ \widehat{A}\widehat{A}^T = I_n \ \mbox{ and }\ \widehat{S}\widehat{A}^T = \begin{bmatrix} SV\Sigma D\\ \sqrt{\lambda}UD\end{bmatrix} = \begin{bmatrix} SU_1\\U_2\end{bmatrix},
\end{equation*}
so that $U_1$ is the first $d$ rows of an orthogonal basis for $\begin{bmatrix}A^T\\ \sqrt{\lambda} I_n \end{bmatrix}$ as required by the theorem. We have the following equality:
\begin{equation*}
    \frac{1}{2}\lscost{A^T\nu}{2}^2 + \frac{1}{2}\lscost{\nu}{2}^2 - \langle b,\ \nu \rangle = \frac{1}{2}\lscost{\widehat{A}^Tw}{2}^2 - \langle DU^Tb,\ w\rangle,
\end{equation*}
for $\left\{\forall \nu \in\reals{n}\ |\ w = D^{-1}U^T\nu \right\}$. Thus, following HS sub-problem is equivalent to \cref{eq:dual_mihs1}
\begin{equation*}
    \Delta w^{i+1} = \swrite{argmin}{y} \lscost{\widehat{S}\widehat{A}^Tw}{2}^2 - 2\langle DU^Tb -  \widehat{A}\widehat{A}^Tw^i, \ w \rangle.
\end{equation*}
We can analyze the following bipartite transformation to figure out the convergence properties of the \ff{Dual M-IHS}
\begin{equation*}
    \begin{bmatrix}
    w^{i+1} - w^* \\
    w^{i} - w^*
    \end{bmatrix} = \underbrace{\begin{bmatrix}
    (1+\beta)I_n - \alpha (\widehat{A}\widehat{S}^T\widehat{S}\widehat{A}^T)^{-1} & -\beta I_n\\
    I_n & \mathbf{0}
    \end{bmatrix}}_{T} \begin{bmatrix}
    w^{i} - w^* \\
    w^{i-1} - w^*
    \end{bmatrix},
\end{equation*}
where $w^* = D^{-1}U^Tv^*$. The rest of the proof can be completed straightforwardly by following the same analysis steps as in the proof for the \ff{M-IHS} case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of the Condition in \cref{lemma:mihs_conv}}\label{proof:cor_sketch}
\Cref{lemma:mihs_conv} is valid if the sketch matrix $S$ satisfies the following condition:
\begin{equation}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2} \leq \lscost{U_1^TS^TSU_1 - U_1^TU_1}{F} \leq \epsilon, \label{eq:aim}
\end{equation}
where
\begin{equation*}
    \lscost{U_1}{F}^2 = \lscost{U\Sigma D}{F}^2 = \lscost{\Sigma(\Sigma^2 +\lambda I_r)^{-1/2}}{F}^2 = \sum\limits_{i=1}^{r}\frac{\sigma_i^2}{\sigma_i^2 + \lambda} = \sd(A),
\end{equation*}
and $\lscost{U_1}{2}^2 = \frac{\sigma_1^2}{\sigma_1^2 + \lambda} \approx 1$ for a properly chosen regularization parameter $\lambda$. If the sketch matrix $S$ is drawn from a randomized distribution $\D$ over matrices $\realss{m}{n}$, then the condition in \cref{eq:aim} can be met with a desired level of probability. For this purpose will use Approximate Matrix Property (AMM) which is given below.
\begin{theorem}\label{theorem:amm_ose}($(\epsilon, \delta, k)$-AMM Property \cite{ref:cnw15_optimal_stable_rank}) If a distribution $\D$ over $S\in\realss{m}{n}$ has the $(\epsilon, \delta, 2k,\ell)$-OSE moment property for some $\delta <1/2$ and $\ell\geq2$, then for any $A,B$:
$$
\prob{S\sim\D}{\lscost{A^TS^TSB - A^TB}{2} > \epsilon\sqrt{\left(\lscost{A}{2}^2+ \frac{\lscost{A}{F}^2}{k}\right)\left(\lscost{B}{2}^2 + \frac{\lscost{B}{F}^2}{k}\right)}} < \delta.
$$
\end{theorem}
The definition of OSE-moment property can be found in \cite{ref:cnw15_optimal_stable_rank}. By \cref{theorem:amm_ose}, the sketch sizes can be chosen in accordance with the embedding size $k$ to satisfy the condition in \cref{eq:aim} as we will show next.

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item1}} Count Sketch with a single nonzero element in each column and size $m\geq 2/({\epsilon'}^2\delta)$ has $(\epsilon', \delta,2)$-JL moment property \cite{ref:tz12}. JL-Moment Property can be found in Definition 6.1 of \cite{ref:kn14_sparser_jl}. By Theorem 6.2 in \cite{ref:kn14_sparser_jl}:
\begin{equation*}
    \lscost{U_1S^TSU_1 - U_1^TU_1}{F} < 3\epsilon'\lscost{U_1}{F}^2 = 3\epsilon'\sd(A) \leq \epsilon
\end{equation*}
for $\epsilon' = \epsilon/(3\sd(A))$. So, condition in \cref{eq:aim} holds with probability at least $1-\delta$, if $m = O(\sd(A)^2/(\epsilon^2\delta))$. 

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item2}} Combining Theorem 4.2 of \cite{ref:coh16_nearly_tight} and Remark 2 of \cite{ref:cnw15_optimal_stable_rank} implies that any sketch matrix drawn from an OSNAP \cite{ref:nn13_osnap} with the conditions given in the item $(ii)$ of \cref{corollary:sketch} satisfies the $(\epsilon', \delta, k, \log(k/\delta))$-OSE moment property thus the $(\epsilon', \delta, k/2)$-AMM Property. Setting $A=B=U_1$  and $k = \sd(A)/2$ in \cref{theorem:amm_ose} gives:
\begin{equation*}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2} \leq \epsilon'(\lscost{U_1}{2}^2 + 2) \leq 3 \epsilon' \leq \epsilon
\end{equation*}
with probability at least $1-\delta$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}
Based on the lower bounds established for any OSE in \cite{ref:nn14_lower}, the Conjecture 14 in \cite{ref:nn13_osnap} states that any OSNAP with 
$m=\Omega((k+\log(1/\delta))/\epsilon^2)$ and 
$s=\Omega(\log(k/\delta)/\epsilon)$ have the $(\epsilon,\delta,k,\ell)$-OSE moment property for $\ell = \Theta(\log(k/\delta))$, an even integer. As a result of the conjecture and \cref{theorem:amm_ose}, the condition in \cref{eq:aim} can be satisfied with probability at least $1-\delta$ by using an OSNAP matrix with size $m=\Omega((\sd(A)+\log(1/\delta))/\epsilon^2)$ and sparsity $s=\Omega(\log(\sd(A)/\delta)/\epsilon)$.
\end{remark}
\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item3}} By Theorem 9 of \cite{ref:cnw15_optimal_stable_rank}, SRHT with the sketch size given in item $(iii)$ has the $(\epsilon', \delta, 2\sd(A), \log(\sd(A)/\delta))$-OSE moment property and thus by \cref{theorem:amm_ose}, it provides $(\epsilon', \delta, \sd(A))$-AMM property. Again, setting $A=B=U_1$ and $k=\sd(A)$ produces the desired result.

\paragraph{\textbf{Proof of Corollary 3.2}, \cref{item4}} The Subgaussian matrices having entries with mean zero and variance $1/m$ satisfy the JL Lemma \cite{ref:jl_lemma} with optimal sketch size \cite{ref:kn14_sparser_jl}. Also, they have the $(\epsilon/2, \delta, \Theta(\log(1/\delta)))$-JL moment property \cite{ref:kmn_11_almost_optimal}. Thus by Lemma 4 of \cite{ref:cnw15_optimal_stable_rank} such matrices have $(\epsilon,\delta,k,\Theta(k+\log(1/\delta)))$-OSE moment property for $\delta < 9^{-k}$, which means $m=\Omega(k/\epsilon^2)$. Again, by setting $A=B=U_1$ and $k = \sd(A)$ in \cref{theorem:amm_ose} gives the desired result.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence proof without regularization} \label{proof:no_reg}
If the LS problem without any regularization is tried to be solved, then we need the following inequality to hold:
\begin{equation*}
    \lscost{U_1^TS^TSU_1 - U_1^TU_1}{2}\leq \epsilon \xRightarrow[n\geq d]{\quad\lambda\to0\quad }\lscost{U^TS^TSU - I_r}{2}\leq \epsilon,
\end{equation*}
which can be satisfied with a constant probability, if the sketch matrix is drawn from a distribution $\D$ that has the OSE Moment property defined in \cref{def:ose_moment}. Then, the bound for the sketch size can be derived by using the other results presented above. The details of how to obtain the above inequality can be found in \cite{ref:mihs}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of \cref{corollary:empirical}} \label{proof:empirical}
Consider the regularized LS solution with parameter $\lambda$ and the Truncated SVD solution with parameter $\lceil\sd(A)\rceil$:
\begin{equation*}
    x^* = \sum\limits_{i=1}^r \frac{\sigma_i^2}{\sigma_i^2 + \lambda}\frac{u_i^Tb}{\sigma_i}v_i \quad\mbox{ and }\quad x^\dagger = \sum\limits_{i=1}^{\lceil\sd(A)\rceil}\frac{u_i^Tb}{\sigma_i}v_i
\end{equation*}
where $u_i$'s and $v_i$'s are columns of $U$ and $V$ matrices in the SVD. The Tikhonov regularization with the closed form solution is preferred in practise to avoid the high computational cost of the SVD. The filtering coefficients of the Tikhonov regularization, $\frac{\sigma_i^2}{\sigma_i^2 + \lambda}$, become very close to the binary filtering coefficients of the TSVD, as the decay rate of the singular values of $A$ increases. In these cases, both the solution $x^*$ and $x^\dagger$ become almost indistinguishable. Thereby, the diagonal matrix, $\Sigma D$, which is used in the proof of \cref{corollary:sketch} can be approximated by the diagonal matrix $\Pi$ where
\begin{equation*}
    \Pi_{ii} = \left\{
\begin{array}{rl}
1 & \text{if } i \leq \sd(A) \leq r\\
0 &  otherwise
\end{array} \right.,
\end{equation*}
which is equivalent to replace the Tikhonov coefficients by the binary TSVD coefficients. Then, we have
\begin{align*}
    \left(\widehat{A}^T\widehat{S}^T\widehat{S}\widehat{A}\right)^{-1} &= \left(D\Sigma U^TS^TSU\Sigma D + \lambda D^2\right)^{-1}\\ &\approx \left(\Pi (SU)^T(SU)\Pi + I_r - \Pi\right)^{-1} = \left[\begin{array}{c|c}
        \widebar{S}^T\widebar{S}& \textbf{0}\\
        \hline
        \textbf{0} & I_{(r - \sd(A))}
    \end{array}\right],
\end{align*}
where $\widebar{S} = SU\Pi\in\realss{m}{\sd(A)}$ has the same distribution as $S$, since $U\Pi$ is an orthonormal transformation. By the Marchenko Pastur Law, the minimum and the maximum eigenvalues of this approximation converge to $\left(1 \pm \sqrt{\frac{\sd(A)}{m}}\right)^{-2}$ as $m\to \infty$ and while $\sd(A)/m$ remains constant \cite{ref:edelman2, ref:edelman}. The rest of the proof follows from the analysis given in \cref{proof:lemma_conv}.
